Long live The NMSSM!

We analyze the scenario within the Next to Minimal Supersymmetric Standard Model (NMSSM), where the lightest supersymmetric particle (LSP) is singlino-like neutralino. By systematically considering various possible admixtures in the electroweakino sector, we classify regions of parameter space where the next to lightest supersymmetric particle (NLSP) is a long-lived electroweakino while remaining consistent with constraints from flavor physics, dark matter direct detection, and collider data. We identify viable cascade decay modes featuring the long-lived NLSP for directly produced chargino-neutralino pairs, thus, leading to displaced vertex signatures at the high luminosity LHC (HL-LHC). We construct track based analysis in order to uncover such scenarios at the HL-LHC and analyze their discovery potential. We show that through such focused searches for the long-lived particles at the HL-LHC, one can probe regions of the electroweakino parameter space that are otherwise challenging.

==> Long live The NMSSM!/header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{makecell}
\newcommand{\myrotcell}[1]{\rotcell{\makebox[0pt][l]{#1}}}
\usepackage{caption, subcaption}  % needed for figures
\usepackage{dcolumn}   % needed for some tables
\usepackage{amsmath, amssymb}        % for math
\usepackage{color,latexsym, array,multirow,  verbatim, enumerate,cancel}
\usepackage{enumitem}
\usepackage{slashed}
\usepackage{bigcenter}
\usepackage{arydshln}
%\usepackage[utf8]{inputenc}
\usepackage[utf8x]{inputenc}
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}
\usepackage[normalem]{ulem}
\usepackage{scalerel}

%\usepackage{subfigure}

\newcommand{\suchita}[1]{\textcolor{red}{Suchita: #1}}
\newcommand{\ad}[1]{\textcolor{red}{Suchita: #1}}
\newcommand{\rkb}[1]{\textcolor{red}{Suchita: #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\issue(#1,#2,#3){{\bf #1}, #2 (#3)}
\def\BibTeX{\rm B{\sc ib}\TeX}
\def\hldg#1{\textcolor{magenta}{\large\textsf{#1}}}
\def\comment#1{\textcolor{blue}{\large(\it{#1})}}
\catcode`\@=11
\def\lsim{\mathrel{\mathpalette\@versim<}}
\def\gsim{\mathrel{\mathpalette\@versim>}}
\def\@versim#1#2{\vcenter{\offinterlineskip
\ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr\sim\crcr } }}
\catcode`\@=12
\def\baselinestretch{1.20}
\parskip 5pt plus 1pt
\catcode`@=12

\newcommand{\met}{$\slashed{E}_T$}


\newcommand{\newc}{\newcommand}
\newc{\wt}{\widetilde}
\newc{\ra}{\rightarrow}

\def\beq {\begin{equation}}
\def\eeq {\end{equation}}
\def\bi {\begin{itemize}}
\def\ei {\end{itemize}}
\def\bea {\begin{eqnarray}}
\def\eea {\end{eqnarray}}
\def \PMET{\rm p{\!\!\!/}_T}
\def \met{\slashed{E}_T}
\def\dkg#1{\textcolor{red}{\large\textsf{#1}}}
\def\ac#1{\textcolor{blue}{\textsf{#1}}}     % amit
\def\comment#1{\textcolor{blue}{\large\textsf{#1}}}
\def \PMETV{\overrightarrow{\rm p}{\!\!\!\!/}_T}
\newcommand{\br}{\begin{eqnarray}}
\newcommand{\er}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\as}{\alpha_s}
\newcommand{\gl}{\widetilde g}
\newcommand{\sq}{\widetilde q}
\newcommand{\ch}{\widetilde \chi^\pm}
\newcommand{\nut}{\widetilde\chi^0}
\newcommand{\stau}{\widetilde\tau}
\newcommand{\aem}{\alpha_{em}}
\newcommand{\st}{\widetilde t}
\def\lum             {{\cal L}}
\newcommand{\ifb} {\rm {fb}^{-1}}

\def\chisq{\chi^2}
\def\chimin{\chi^2_{\rm min}}


\def \chii {{\wt\chi_i}}
\def \chij {{\wt\chi_j}}
%----------------------------------------------------
% Chargino
\def \charginopm{{\wt\chi}^{\pm}}
\def \mcharginopm{m_{\charginopm}}
\def \chonep {{\wt\chi_1^+}}
\def \chone {{\wt\chi_1}}
\def \ch2p {{\wt\chi_2^+}}
\def \chonem {{\wt\chi_1^-}}
\def \ch2m {{\wt\chi_2^-}}
\def \chplus {{\wt\chi^+}}
\def \chminus {{\wt\chi^-}}
\def \chip{{\wt\chi_i}^{+}}
\def \chim{{\wt\chi_i}^{-}}
\def \chipm{{\wt\chi_i}^{\pm}}
\def \chjp{{\wt\chi_j}^{+}}
\def \chjm{{\wt\chi_j}^{-}}
\def \chjpm{{\wt\chi_j}^{\pm}}
\def \chonepm{{\wt\chi_1}^{\pm}}
\def \chonemp{{\wt\chi_1}^{\mp}}
\def \mchonepm{m_{\chonepm}}
\def \mchonemp{m_{\chonemp}}
\def \mchtwopm{m_{\chtwopm}}
\newc{\dmchi}{\Delta m_{\wt\chi}}
\def \chtwop {{\wt\chi_2^+}}
\def \chtwom {{\wt\chi_2^-}}
\def \chtwopm{{\wt\chi_2}^{\pm}}
\def \chtwomp{{\wt\chi_2}^{\mp}}

\def \chkpm{{\wt\chi_k}^{\pm}}
\def \chkmp{{\wt\chi_k}^{\mp}}
\def \chlpm{{\wt\chi_\ell}^{\pm}}
\def \chlmp{{\wt\chi_\ell}^{\mp}}
%-----------------------------------------------------------------------
% Neutralino
\def \lsp{\wt\chi_1^0}
\def \vlsp{\emph{VLSP}}
\def \lspi{\wt\chi_i^0}
\def \mlspi{m_{\lspi}}
\def \lspj{\wt\chi_j^0}
\def \mlspj{m_{\lspj}}
\def \lspone{\wt\chi_1^0}
\def \mlspone{m_{\lspone}}
\def \lsptwo{\wt\chi_2^0}
\def \lspthreefour{\wt\chi_{3,4}^0}
\def \lsponetwo{\wt\chi_{1,2}^0}
\def \mlsptwo{m_{\lsptwo}}
\def \lspthree{\wt\chi_3^0}
\def \mlspthree{m_{\lspthree}}
\def \lspfour{\wt\chi_4^0}
\def \mlspfour{m_{\lspfour}}
\def \lspfive{\wt\chi_5^0}
\def \mlspfive{m_{\lspfive}}
\def \slep{\wt{l}}
\def \mslep{m_{\slep}}
\def \stauone{\wt\tau_1}
\def \mstauone{m_{\stauone}}
%-----------------------------------------------------------------------
\def\tcr{\textcolor{red}}
\def\tcg{\textcolor{green}}
\def\tcb{\textcolor{blue}}
\def\tcm{\textcolor{magenta}}
\def\amit{\textcolor{magenta}}
\def\rkb{\textcolor{blue}}

\def\issue(#1,#2,#3){{\bf #1}, #2 (#3)}

\hypersetup{
   colorlinks=true,       % false: boxed links; true: colored links
   linkcolor=blue,        % color of internal links
   citecolor=blue,         % color of links to bibliography
   filecolor=magenta,      % color of file links
   }

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}


\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}

%Ref Style
\bibliographystyle{utphys}


==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{makecell}
\newcommand{\myrotcell}[1]{\rotcell{\makebox[0pt][l]{#1}}}
\usepackage{caption, subcaption}  % needed for figures
\usepackage{dcolumn}   % needed for some tables
\usepackage{amsmath, amssymb}        % for math
\usepackage{color,latexsym, array,multirow,  verbatim, enumerate,cancel}
\usepackage{enumitem}
\usepackage{slashed}
\usepackage{bigcenter}
\usepackage{arydshln}
%\usepackage[utf8]{inputenc}
\usepackage[utf8x]{inputenc}
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}
\usepackage[normalem]{ulem}
\usepackage{scalerel}

%\usepackage{subfigure}

\newcommand{\suchita}[1]{\textcolor{red}{Suchita: #1}}
\newcommand{\ad}[1]{\textcolor{red}{Suchita: #1}}
\newcommand{\rkb}[1]{\textcolor{red}{Suchita: #1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\issue(#1,#2,#3){{\bf #1}, #2 (#3)}
\def\BibTeX{\rm B{\sc ib}\TeX}
\def\hldg#1{\textcolor{magenta}{\large\textsf{#1}}}
\def\comment#1{\textcolor{blue}{\large(\it{#1})}}
\catcode`\@=11
\def\lsim{\mathrel{\mathpalette\@versim<}}
\def\gsim{\mathrel{\mathpalette\@versim>}}
\def\@versim#1#2{\vcenter{\offinterlineskip
\ialign{$\m@th#1\hfil##\hfil$\crcr#2\crcr\sim\crcr } }}
\catcode`\@=12
\def\baselinestretch{1.20}
\parskip 5pt plus 1pt
\catcode`@=12

\newcommand{\met}{$\slashed{E}_T$}


\newcommand{\newc}{\newcommand}
\newc{\wt}{\widetilde}
\newc{\ra}{\rightarrow}

\def\beq {\begin{equation}}
\def\eeq {\end{equation}}
\def\bi {\begin{itemize}}
\def\ei {\end{itemize}}
\def\bea {\begin{eqnarray}}
\def\eea {\end{eqnarray}}
\def \PMET{\rm p{\!\!\!/}_T}
\def \met{\slashed{E}_T}
\def\dkg#1{\textcolor{red}{\large\textsf{#1}}}
\def\ac#1{\textcolor{blue}{\textsf{#1}}}     % amit
\def\comment#1{\textcolor{blue}{\large\textsf{#1}}}
\def \PMETV{\overrightarrow{\rm p}{\!\!\!\!/}_T}
\newcommand{\br}{\begin{eqnarray}}
\newcommand{\er}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\as}{\alpha_s}
\newcommand{\gl}{\widetilde g}
\newcommand{\sq}{\widetilde q}
\newcommand{\ch}{\widetilde \chi^\pm}
\newcommand{\nut}{\widetilde\chi^0}
\newcommand{\stau}{\widetilde\tau}
\newcommand{\aem}{\alpha_{em}}
\newcommand{\st}{\widetilde t}
\def\lum             {{\cal L}}
\newcommand{\ifb} {\rm {fb}^{-1}}

\def\chisq{\chi^2}
\def\chimin{\chi^2_{\rm min}}


\def \chii {{\wt\chi_i}}
\def \chij {{\wt\chi_j}}
%----------------------------------------------------
% Chargino
\def \charginopm{{\wt\chi}^{\pm}}
\def \mcharginopm{m_{\charginopm}}
\def \chonep {{\wt\chi_1^+}}
\def \chone {{\wt\chi_1}}
\def \ch2p {{\wt\chi_2^+}}
\def \chonem {{\wt\chi_1^-}}
\def \ch2m {{\wt\chi_2^-}}
\def \chplus {{\wt\chi^+}}
\def \chminus {{\wt\chi^-}}
\def \chip{{\wt\chi_i}^{+}}
\def \chim{{\wt\chi_i}^{-}}
\def \chipm{{\wt\chi_i}^{\pm}}
\def \chjp{{\wt\chi_j}^{+}}
\def \chjm{{\wt\chi_j}^{-}}
\def \chjpm{{\wt\chi_j}^{\pm}}
\def \chonepm{{\wt\chi_1}^{\pm}}
\def \chonemp{{\wt\chi_1}^{\mp}}
\def \mchonepm{m_{\chonepm}}
\def \mchonemp{m_{\chonemp}}
\def \mchtwopm{m_{\chtwopm}}
\newc{\dmchi}{\Delta m_{\wt\chi}}
\def \chtwop {{\wt\chi_2^+}}
\def \chtwom {{\wt\chi_2^-}}
\def \chtwopm{{\wt\chi_2}^{\pm}}
\def \chtwomp{{\wt\chi_2}^{\mp}}

\def \chkpm{{\wt\chi_k}^{\pm}}
\def \chkmp{{\wt\chi_k}^{\mp}}
\def \chlpm{{\wt\chi_\ell}^{\pm}}
\def \chlmp{{\wt\chi_\ell}^{\mp}}
%-----------------------------------------------------------------------
% Neutralino
\def \lsp{\wt\chi_1^0}
\def \vlsp{\emph{VLSP}}
\def \lspi{\wt\chi_i^0}
\def \mlspi{m_{\lspi}}
\def \lspj{\wt\chi_j^0}
\def \mlspj{m_{\lspj}}
\def \lspone{\wt\chi_1^0}
\def \mlspone{m_{\lspone}}
\def \lsptwo{\wt\chi_2^0}
\def \lspthreefour{\wt\chi_{3,4}^0}
\def \lsponetwo{\wt\chi_{1,2}^0}
\def \mlsptwo{m_{\lsptwo}}
\def \lspthree{\wt\chi_3^0}
\def \mlspthree{m_{\lspthree}}
\def \lspfour{\wt\chi_4^0}
\def \mlspfour{m_{\lspfour}}
\def \lspfive{\wt\chi_5^0}
\def \mlspfive{m_{\lspfive}}
\def \slep{\wt{l}}
\def \mslep{m_{\slep}}
\def \stauone{\wt\tau_1}
\def \mstauone{m_{\stauone}}
%-----------------------------------------------------------------------
\def\tcr{\textcolor{red}}
\def\tcg{\textcolor{green}}
\def\tcb{\textcolor{blue}}
\def\tcm{\textcolor{magenta}}
\def\amit{\textcolor{magenta}}
\def\rkb{\textcolor{blue}}

\def\issue(#1,#2,#3){{\bf #1}, #2 (#3)}

\hypersetup{
   colorlinks=true,       % false: boxed links; true: colored links
   linkcolor=blue,        % color of internal links
   citecolor=blue,         % color of links to bibliography
   filecolor=magenta,      % color of file links
   }

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}


\renewcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}

%Ref Style
\bibliographystyle{utphys}

